Sparsity-Accelerated Training for Large Language Models

Large language models (LLMs) have demonstrated proficiency across various natural language processing (NLP) tasks but often require additional training, such as continual pre-training and supervised fine-tuning. However, the costs associated with this, primarily due to their large parameter count, remain high. This paper proposes leveraging \emph{sparsity} in pre-trained LLMs to expedite this training process. By observing sparsity in activated neurons during forward iterations, we identify the potential for computational speed-ups by excluding inactive neurons. We address associated challenges by extending existing neuron importance evaluation metrics and introducing a ladder omission rate scheduler. Our experiments on Llama-2 demonstrate that Sparsity-Accelerated Training (SAT) achieves comparable or superior performance to standard training while significantly accelerating the process. Specifically, SAT achieves a $45\%$ throughput improvement in continual pre-training and saves $38\%$ training time in supervised fine-tuning in practice. It offers a simple, hardware-agnostic, and easily deployable framework for additional LLM training. Our code is available at https://github.com/OpenDFM/SAT.

==> sections/7.ethics.tex <==
\section*{Ethics Statement}
No ethical issues are involved in this work since all datasets and models adopted in this paper are publicly available and along with bibliographic citations. 

==> tables/ct-data.tex <==
% \usepackage{multirow}
% \usepackage{arydshln}


\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccc|cccc|c|} 
\hline

\hline
%--------------------------------------------------------
\multirow{2}{*}{Dataset} & \multicolumn{4}{c|}{English} & \multicolumn{4}{c|}{Chinese} & \multicolumn{1}{c|}{Code} \\
\cdashline{2-5}
& Arxiv & Books & StackExchange & Wiki & Baike & Wiki & WuDao & Others & Github\\
\hline
\#Tokens~(B) & 0.1 \\

\hline

\hline
\end{tabular}
}
\end{table*}

